Objects as volumes: A stochastic geometry view of opaque solids

We develop a theory for the representation of opaque solids as volumes. Starting from a stochastic representation of opaque solids as random indicator functions, we prove the conditions under which such solids can be modeled using exponential volumetric transport. We also derive expressions for the volumetric attenuation coefficient as a functional of the probability distributions of the underlying indicator functions. We generalize our theory to account for isotropic and anisotropic scattering at different parts of the solid, and for representations of opaque solids as stochastic implicit surfaces. We derive our volumetric representation from first principles, which ensures that it satisfies physical constraints such as reciprocity and reversibility. We use our theory to explain, compare, and correct previous volumetric representations, as well as propose meaningful extensions that lead to improved performance in 3D reconstruction tasks.

==> integration.tex <==
\section{Numerical Integration}\label{sec:numerical_integration} 

We use quadrature~\eqref{eqn:emissive_only_volume_quadrature} to estimate the emission-only volume rendering equation~\eqref{eqn:emissive_only_volume}. The specific variety of quadrature we use was introduced by~\citet{max1995optical} and recently popularized by~\citet{mildenhall2021nerf}. Readers familiar with this technique may skip this section. We provide a derivation here as an anchoring point for our comparison with UNISURF~\citep{oechsle2021unisurf}.

In practice, most neural volume rendering pipelines learn an emission function which for simplicity we write as $\emission\paren{\point, \direction}$. Incorporating this emission function into the emission-only volume rendering equation (Equation (7) of main paper) gives us:
% 
\begin{equation}
    L\paren{\point, \direction} = \int_{\distance_n}^{\distance_f} \freeflight_{\point, \direction}\paren{\distanceVariable} \emission\paren{\ray_{\point,\direction}(\distanceVariable), -\direction}\ud \distanceVariable \label{eqn:emissive_only_volume}
\end{equation}
%
We note that the bounds of the integral $\distance_n$ and $\distance_f$ denote a near and far plane. Additionally, in our theory $\Exp{\geometry}{L_i\paren{\point, \direction}} = L\paren{\point, \direction}$ and $\emission\paren{\ray_{\point,\direction}(\distanceVariable), -\direction} = \Exp{\geometry}{L_o\paren{\ray_{\point, \direction}\paren{\distance}, -\direction}}$. Our derivation below assumes exponential transport.%We will, however, use the more general notation for this section since the numerical integration technique we discuss applies to any volume rendering equation involving exponential transmittance.

We begin by selecting $N$ points along a ray $\ray_{x,\direction}\paren{\distanceVariable_0}, \ray_{x,\direction}\paren{\distanceVariable_1}, \hdots, \ray_{x,\direction}\paren{\distanceVariable_N}$ and then divide the ray into $N$ intervals $[\distance_i, \distance_{i+1}]$. The intervals are chosen such that they partition the ray 
%
\begin{equation}
	[\distance_n, \distance_f] = [\distance_1, \distance_2] \cup [\distance_2, \distance_3] \cup \hdots \cup[\distance_{N}, \distance_{N+1}]
\end{equation}
%
and each point belongs to exactly one interval $s_i\in[\distance_i, \distance_{i+1}]$. The most naive approach is to uniformly sample $N$ points and then choose the bounds of the intervals such that they are equidistant from neighboring points. We additionally simplify our derivations by indexing the points and intervals such that they have a straightforward ordering 
%
\begin{gather}
	s_1 < s_2 < \hdots < s_N\\
	t_1 < t_2 < \hdots < t_{N+1}
\end{gather}
%
The quadrature technique we derive assumes both $\emission\paren{\ray_{\point,\direction}(\distanceVariable), -\direction}$ and $\coeff\paren{\ray_{\point,\direction}(\distanceVariable), \direction}$ are approximately constant functions of $s$ within any interval $[\distance_i, \distance_{i+1}]$ of the ray. Under this assumption, we can approximate the volume rendering equation~\eqref{eqn:emissive_only_volume} as
%
\begin{gather}
L\paren{\point, \direction}
    \approx \sum_{i=1}^N \transmittanceEstimate_{\point, \direction}\paren{\distance_i} \absorptionEstimate_{\point,\direction}(\distance_i,\distance_{i+1})\emission\paren{\ray_{\point,\direction}(\distanceVariable_i), -\direction}\label{eqn:emissive_only_volume_quadrature}\\
\transmittanceEstimate_{\point, \direction}\paren{\distance_i} = \prod_{j=0}^{i-1} \transmittanceEstimate_{\point,\direction}\paren{\distance_{j}, \distance_{j+1}}\\
\transmittanceEstimate_{\point, \direction}\paren{\distance_i,\distance_{i+1}} = \exp\paren{-\coeff\paren{\ray_{\point,\direction}\paren{s_i}} |\distance_{i+1} - \distance_i|}\\
\absorptionEstimate_{\point, \direction}\paren{\distance_i,\distance_{i+1}} = 1 - \transmittanceEstimate_{\point, \direction}\paren{\distance_i,\distance_{i+1}}
\end{gather}
%
In the following, we derive the above expression. %We first rewrite~\eqref{eqn:emissive_only_volume} under the assumption that~$\emission$ is constant within each interval and then we'll derive approximations for transmittance by assuming $\coeff$ is constant within each interval.

\paragraph{Approximating emission.} By treating the emission function as constant along each interval $[\distance_i,\distance_{i+1}]$, equation~\eqref{eqn:emissive_only_volume} reduces to a form more amenable to evaluation.
%
\begin{align}
L\paren{\point, \direction} 
    &= \int_0^\distance \freeflight_{\point, \direction}\paren{\distanceVariable} \emission\paren{\ray_{\point,\direction}(\distanceVariable), -\direction}\ud \distanceVariable\\
     &= \sum_{i=1}^N \int_{\distance_i}^{\distance_{i+1}} \freeflight_{\point, \direction}\paren{\distanceVariable} \emission\paren{\ray_{\point,\direction}(\distanceVariable), -\direction}\ud \distanceVariable\\
     &\approx\sum_{i=1}^N \emission\paren{\ray_{\point,\direction}(\distanceVariable_i), -\direction}\int_{\distance_i}^{\distance_{i+1}} \freeflight_{\point, \direction}\paren{\distanceVariable} \ud \distanceVariable.
\end{align}
%
The integral of the free-flight PDF over the segment can now be evaluated which reveals an intuitive expression depending only on transmittance.
\begin{align}
&\int_{\distance_i}^{\distance_{i+1}} \freeflight_{\point, \direction}\paren{\distanceVariable} \ud\distanceVariable=\int_{\distance_i}^{\distance_{i+1}} \transmittance_{\point, \direction}\paren{\distanceVariable} \coeff_{\point,\direction}\paren{\ray_{\point,\direction}\paren{\distanceVariable}, \direction}\ud\distanceVariable\\
&\hspace{4ex}=\transmittance_{\point, \direction}\paren{\distance_i} \int_{\distance_i}^{\distance_{i+1}} \transmittance_{\point, \direction}\paren{\distance_i,\distanceVariable}\coeff_{\point,\direction}\paren{\ray_{\point,\direction}\paren{\distanceVariable}, \direction}\ud\distanceVariable\\
&\hspace{4ex}=\transmittance_{\point, \direction}\paren{\distance_i} \paren{1-\transmittance_{\point,\direction}(\distance_i,\distance_{i+1})}\\
&\hspace{4ex}=\transmittance_{\point, \direction}\paren{\distance_i} \absorption_{\point,\direction}(\distance_i,\distance_{i+1})\label{eqn:free_flight_segment}
\end{align}
%
Above, we implicitly introduce the following notation for both transmittance through and absorption within any given interval.
%
\begin{align}
\transmittance_{\point, \direction}\paren{\distance_i, \distance_{i+1}} &= \exp\paren{-\int_{\distance_i}^{\distance_{i+1}} \coeff\paren{\ray_{\point,\direction}\paren{\distanceVariable}, \direction} \ud \distanceVariable}\\
\absorption_{\point, \direction}\paren{\distance_i, \distance_{i+1}} &= 1 - \transmittance_{\point, \direction}\paren{\distance_i, \distance_{i+1}}
\end{align}
%
Equation~\eqref{eqn:free_flight_segment} allows us to write the volume rendering equation in terms of only transmittance and the emission function.
%
\begin{equation}
L\paren{\point, \direction} 
    \approx\sum_{i=1}^n \transmittance_{\point, \direction}\paren{\distance_i} \absorption_{\point,\direction}(\distance_i,\distance_{i+1})\emission\paren{\ray_{\point,\direction}(\distanceVariable_i), -\direction}\label{eqn:emissive_only_volume_alternative}
\end{equation}

\paragraph{Approximating transmittance.} Exponential transmittance has an analytic expression when the extinction coefficient is a constant, say $\overline{\coeff}$.
%
\begin{equation}
\transmittance\paren{\distance} 
= \exp\paren{-\int_{0}^{t} \overline{\coeff} \ud \distanceVariable}
= \exp\paren{- \overline{\coeff} t}
\end{equation}
%
Since we assume that $\coeff\paren{\ray_{\point,\direction}(\distanceVariable), \direction}$ is constant along intervals of a ray, we can use this closed-form expression. On any given interval of the ray $[\distance_i,\distance_{i+1}]$ we substitute $\coeff\paren{\ray_{\point,\direction}(\distanceVariable_i), \direction}$ in place of a constant $\overline{\coeff}$
%
\begin{equation}
\transmittanceEstimate_{\point,\direction}\paren{\distance_i, \distance_{i+1}}= \exp\paren{-\coeff\paren{\ray_{\point,\direction}\paren{\distanceVariable_i}, \direction} |\distance_{i+1} - \distance_{i}|}\label{eq:approximate_segment_transmittance}\\
\end{equation}
%
We also write $\transmittanceEstimate$ rather than $\transmittance$ to emphasize the fact that we are evaluating transmittance analytically. As absorption along an interval is defined in terms of transmittance, we similarly use $\overline{\absorption}$ to emphasize that the absorption within the segment is computed using analytic transmittance functions. 
%
\begin{equation}
\absorptionEstimate_{\point,\direction}\paren{\distance_i,\distance_{i+1}}
= 1 -\transmittanceEstimate_{\point,\direction}\paren{\distance_i, \distance_{i+1}}
\end{equation}
%
Although we only have analytic expressions for transmittance along intervals where the extinction coefficient is constant, we can couple these analytic expressions together to evaluate transmittance along the entire ray. In particular, we begin from the definition of transmittance and reformulate it as a product of transmittance along segments.
%
\begin{align}
\transmittance_{\point, \direction}\paren{\distance}
&= \exp\paren{-\int_{\distance_n}^{\distance_f} \coeff\paren{\ray_{\point,\direction}\paren{\distanceVariable}, \direction} \ud \distanceVariable}\\
&= \exp\paren{-\sum_{i=1}^{N} \int_{\distance_i}^{\distance_{i+1}} \coeff\paren{\ray_{\point,\direction}\paren{\distanceVariable}, \direction} \ud \distanceVariable}\\
&= \prod_{i=1}^{N} \exp\paren{-\int_{\distance_i}^{\distance_{i+1}} \coeff\paren{\ray_{\point,\direction}\paren{\distanceVariable}, \direction} \ud \distance}\\
&= \prod_{i=1}^{N} \transmittance_{\point, \direction}\paren{\distance_i, \distance_{i+1}}
\end{align}
%
From this product form of transmittance, we can substitute the analytic expressions for transmittance along each interval to obtain an analytic expression for transmittance along the entire ray.
\begin{align}
\transmittanceEstimate_{\point, \direction}\paren{\distance}
&= \prod_{i=1}^{N-1} \transmittanceEstimate_{\point, \direction}\paren{\distance_i, \distance_{i+1}}
\end{align}
%
Substituting these analytic definitions of transmittance and absorption into equation~\eqref{eqn:emissive_only_volume_alternative} we obtain equation~\eqref{eqn:emissive_only_volume_quadrature}.

==> toc.tex <==
\section{Contents} \label{sec:contents}

The supplementary material has four parts: This supplemental document, an explanatory video (\texttt{supplemental\_video.mp4}), an interactive HTML visualization of our 3D reconstruction results (\texttt{interactive\_visualization}), and code for our implementation (\texttt{code}).

The supplemental document includes the following:
%
\begin{tight_itemize}
	\item In \cref{sec:pointcloud}, we discuss volumetric representations of point clouds, and show additional proof-of-concept experiments on point cloud volume rendering.
	\item In \cref{sec:illumination}, we discuss representations for global illumination, and show additional proof-of-concept experiments on novel-view synthesis.
	\item In \cref{sec:otherprior}, we discuss relationship of our theory to other prior work.
	\item In \cref{sec:implementation}, we discuss implementation details for our 3D reconstruction experiments.
	\item In \cref{sec:quantitative}, we show additional quantitative results for our 3D reconstruction experiments.
	\item In \cref{sec:proofs}, we provide proofs for our theoretical results.
\end{tight_itemize}
